An Algorithm for Illuminating $n$ Nonoverlapping Circular Discs' Boundaries on the Plane with Application to Tree Stem Illumination Problem

Given a set of $n$ nonoverlapping circular discs on a plane, we aim to determine possible positions of points (referred to as cameras) that could fully illuminate all the circular discs' boundaries. This work presents a geometric approach for determining feasible camera positions that would provide total illumination of all circular discs. The Laguerre Delaunay triangulation, coupled with the intersection of slabs formed by the boundaries of circular discs, is employed to form the region that satisfies the given conditions. The experiment is conducted using a set of randomly positioned circular discs on a plane. This study has the potential to address the issue of illumination in forests by utilizing a LiDAR camera to determine the possible number and placement of cameras that can effectively illuminate trees within a forest.

==> scias_macros.tex <==
% macros used in ScienceAsia 
% no copyright
% last updated: 16 Oct 2015

% If you get errors using the commands/environments it is probably
% because the class file you are using has not loaded a necessary package. 
% You can include a package with \usepackage{ } in the preamble.  
% Many of the maths-related commands/environments need
% the amsmath and amssymb packages - you should therefore always
% include these if the class file has not already done so.

% list of packages needed:
% \usepackage{amsmath,amssymb}
% \usepackage{graphicx}
% \usepackage{threeparttable,booktabs}
% \usepackage{url}
% \usepackage[version=3]{mhchem}
% \usepackage{listings}

%% redefine relations
\renewcommand{\leq}{\leqslant}
\renewcommand{\geq}{\geqslant}
\renewcommand{\le}{\leqslant}
\renewcommand{\ge}{\geqslant}
\renewcommand{\ll}{\mathrel{\!<\!\!<\!}} % much less than
\renewcommand{\gg}{\mathrel{\!>\!\!>\!}} % much greater than

%% equations
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bse}{\begin{subequations}}
\newcommand{\ese}{\end{subequations}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\beqas}{\begin{eqnarray*}}
\newcommand{\eeqas}{\end{eqnarray*}}
\def\bml#1\eml{\begin{multline}#1\end{multline}} % suggested in technote.tex
\def\bmls#1\emls{\begin{multline*}#1\end{multline*}}
\def\bal#1\eal{\begin{align}#1\end{align}} % suggested in technote.tex
\def\bals#1\eals{\begin{align*}#1\end{align*}}
\def\bga#1\ega{\begin{gather}#1\end{gather}} % suggested in technote.tex
\def\bgas#1\egas{\begin{gather*}#1\end{gather*}}
\def\bsp#1\esp{\begin{split}#1\end{split}}
\newcommand{\bald}{\begin{aligned}}
\newcommand{\eald}{\end{aligned}}
\newcommand{\bgad}{\begin{gathered}}
\newcommand{\egad}{\end{gathered}}
\newlength{\defaultmultlinegap}
\setlength{\defaultmultlinegap}{\multlinegap}
\newcommand{\zmlg}{\setlength{\multlinegap}{0pt}} % zero multlinegap
\newcommand{\rmlg}{\setlength{\multlinegap}{\defaultmultlinegap}} % restore


% redefine table and table* environments to include threeparttable
\let\oldtable\table
\let\endoldtable\endtable
\renewenvironment{table}[1][tbp]%
{\begin{oldtable}[#1]\relax
\begin{threeparttable}}
{\end{threeparttable}\end{oldtable}}
\expandafter\let\csname oldtablestar\expandafter\endcsname\csname table*\endcsname
\expandafter\let\csname oldendtablestar\expandafter\endcsname\csname endtable*\endcsname
\renewenvironment{table*}[1][tbp]%
{\oldtablestar[#1]\relax\begin{threeparttable}}
{\normalsize\end{threeparttable}\oldendtablestar}

% redefine tnote (threeparttable.sty) so that it doesn't upset alignment
\let\oldtnote\tnote
\renewcommand{\tnote}[1]{\makebox[0pt][l]{\oldtnote{#1}}}

%% figure and table environments
\newcommand{\bfig}{\begin{figure}}
\newcommand{\efig}{\end{figure}}
\newcommand{\bfigs}{\begin{figure*}}
\newcommand{\efigs}{\end{figure*}}
\newcommand{\btab}{\begin{table}}
\newcommand{\etab}{\end{table}}
\newcommand{\btabs}{\begin{table*}}
\newcommand{\etabs}{\end{table*}}

% needs graphicx package
\newcommand{\incgcw}[1]{\includegraphics[width=\columnwidth]{#1}}
\newcommand{\cincgcm}[2]{\centering{\includegraphics[width=#1cm]{#2}}}

% needs booktabs package
\newcommand{\btsf}[1]
{\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}#1}\toprule}
\newcommand{\etsf}{\bottomrule\end{tabular*}}

% needs threeparttable package
\newcommand{\btn}{\begin{tablenotes}}
\newcommand{\etn}{\end{tablenotes}}



\makeatletter
\newif\if@hrefs

%% environments 
\newtheorem{theorem}{Theorem}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{lem}[lemma]{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{cor}[corollary]{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{prop}[proposition]{Proposition}
\newtheorem{identity}{Identity}
\newtheorem{idn}[identity]{Identity}
\newtheorem{@remark}{Remark}
\newenvironment{remark}{\begin{@remark}\upshape}{\end{@remark}}
\newenvironment{rem}{\begin{@remark}\upshape}{\end{@remark}}
\newtheorem{@definition}{Definition}
\newenvironment{definition}{\begin{@definition}\upshape}{\end{@definition}}
\newenvironment{defn}{\begin{@definition}\upshape}{\end{@definition}}
\newtheorem{@example}{Example}
\newenvironment{example}{\begin{@example}\upshape}{\end{@example}}
\newtheorem{@algorithm}{Algorithm}
\newenvironment{algorithm}{\begin{@algorithm}\upshape}{\end{@algorithm}}
\newenvironment{alg}{\begin{@algorithm}\upshape}{\end{@algorithm}}

% needs ifthen package
\newenvironment{proof}[1][]%
{\noindent\textit{\ifthenelse{\equal{#1}{}}{Proof}{Proof #1}}: }%
{\leavevmode\unskip\nobreak\quad\hspace*{\fill}$\Box$\par}
% might be better to omit the \nobreak in the above
% -- it tries to force box not to be on a line on its own
%    which sometimes results in ugly hyphenation

\newcounter{@step}\newcounter{@substep}
\newcommand{\setfirststepnumber}[1]
{\setcounter{@step}{#1}\addtocounter{@step}{-1}}
\newenvironment{steps}{\begin{list}{Step~\arabic{@step}:}
{\setlength{\labelwidth}{-2mm}\setlength{\leftmargin}{6mm}
\setlength{\labelsep}{2mm}\setlength{\itemindent}{-6mm}
\setlength{\listparindent}{6mm}
\setlength{\topsep}{0pt}\setlength{\itemsep}{0ex}\setlength{\parsep}{0ex}
\usecounter{@step}}}
{\end{list}}

% redefine enumerate (intended for use in theorem-like environments only)
\newcounter{@enum}
\renewcommand{\the@enum}{\roman{@enum}}
\renewenvironment{enumerate}{\begin{list}{{\upshape(\the@enum)}}
{\setlength{\labelwidth}{-2mm}\setlength{\leftmargin}{6mm}
\setlength{\labelsep}{2mm}\setlength{\itemindent}{-6mm}
\setlength{\listparindent}{6mm}
\setlength{\topsep}{0pt}\setlength{\itemsep}{0ex}\setlength{\parsep}{0ex}
\usecounter{@enum}}}
{\end{list}}

\newcommand{\ben}{\begin{enumerate}}
\newcommand{\een}{\end{enumerate}}


\newif\if@hrefs

%% labels and references

\newcommand{\elabel}[1]{\label{e:#1}}
\newcommand{\flabel}[1]{\label{f:#1}}
\newcommand{\tlabel}[1]{\label{t:#1}}
\newcommand{\llabel}[1]{\label{l:#1}}
\newcommand{\ilabel}[1]{\label{i:#1}}
\newcommand{\Tlabel}[1]{\label{T:#1}}
\newcommand{\Llabel}[1]{\label{L:#1}}
\newcommand{\Clabel}[1]{\label{C:#1}}
\newcommand{\Plabel}[1]{\label{P:#1}}
\newcommand{\Ilabel}[1]{\label{I:#1}}
\newcommand{\Rlabel}[1]{\label{R:#1}}
\newcommand{\Dlabel}[1]{\label{D:#1}}
\newcommand{\Elabel}[1]{\label{E:#1}}
\newcommand{\Alabel}[1]{\label{A:#1}}
\newcommand{\eref}[1]{\textup{(\ref{e:#1})}}
\newcommand{\eiref}[1]{\textup{(\ref{i:#1})}}
\newcommand{\iref}[1]{\ref{i:#1}}
\newcommand{\fref}[1]{\if@hrefs\mbox{\autoref{f:#1}}\else\mbox{\figurename~\ref{f:#1}}\fi}
\newcommand{\tref}[1]{\if@hrefs\mbox{\autoref{t:#1}}\else\mbox{\tablename~\ref{t:#1}}\fi}
\newcommand{\Tref}[1]{\if@hrefs\autoref{T:#1}\else Theorem~\ref{T:#1}\fi}
\newcommand{\Lref}[1]{\if@hrefs\autoref{L:#1}\else Lemma~\ref{L:#1}\fi}
\newcommand{\Cref}[1]{\if@hrefs\autoref{C:#1}\else Corollary~\ref{C:#1}\fi}
\newcommand{\Pref}[1]{\if@hrefs\autoref{P:#1}\else Proposition~\ref{P:#1}\fi}
\newcommand{\Iref}[1]{\if@hrefs\autoref{I:#1}\else Identity~\ref{I:#1}\fi}
\newcommand{\Rref}[1]{\if@hrefs\autoref{R:#1}\else Remark~\ref{R:#1}\fi}
\newcommand{\Dref}[1]{\if@hrefs\autoref{D:#1}\else Definition~\ref{D:#1}\fi}
\newcommand{\Eref}[1]{\if@hrefs\autoref{E:#1}\else Example~\ref{E:#1}\fi}
\newcommand{\Aref}[1]{\if@hrefs\autoref{A:#1}\else Algorithm~\ref{A:#1}\fi}

%% lstlisting settings - 'numberfirstline=false' is ignored??
\newcommand{\lref}[1]{\if@hrefs\mbox{\autoref{l:#1}}\else\mbox{\lstlistingname~\ref{l:#1}}\fi}
\lstset{xleftmargin=8pt,
  numberfirstline=false,
  numbers=left,numberstyle=\tiny,stepnumber=5,numbersep=4pt,
  basicstyle=\small\ttfamily,commentstyle=\rmfamily,stringstyle=\textsl,
  language={}}

\makeatother

%% fractions
\newcommand{\dsfrac}[2]{\frac{\displaystyle{#1}}{\displaystyle{#2}}} 

%% vectors
\newcommand{\vect}[1]{\boldsymbol{\bf #1}} % need both bf and boldsymbol
\newcommand{\uvect}[1]{\boldsymbol{\bf \hat{#1}}} % unit vector
\newcommand{\spdot}{\,\vect{.}\,}  % scalar product dot
\newcommand{\grad}{\vect{\nabla}}
\renewcommand{\div}{\grad\spdot}
\newcommand{\curl}{\grad\times}

%% differentials and derivatives
\newcommand{\sod}[1]{\,\mathrm{d}#1} % space ordinary differential
\newcommand{\od}[1]{\mathrm{d}#1} % ordinary differential
\newcommand{\fod}[2]{\frac{\mathrm{d} #1}{\mathrm{d} #2}}
\newcommand{\fodn}[3]{\frac{\mathrm{d}^{#3} #1}{\mathrm{d} #2^{#3}}}
\newcommand{\pd}{\partial} % partial differential
\newcommand{\fpd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\fpdn}[3]{\frac{\partial^{#3} #1}{\partial #2^{#3}}}

%% roman superscripts and subscripts
\newcommand{\rs}[1]{_{\mathrm{#1}}} % roman subscript
\newcommand{\rp}[1]{^{\mathrm{#1}}} % roman superscript (p for power)

%% degrees
% should test for presence of textsymbol package
\newcommand{\degree}{\ensuremath{^{\circ}}}
%\newcommand{\degree}{\textdegree}
\newcommand{\Deg}{\operatorname{deg}} % for backwards compatibility
%support is the smallest closed subset of domain where the function is nonzero
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\essinf}{\operatorname*{ess\,inf}}
\newcommand{\argmax}{\operatorname*{arg\,max}}
\newcommand{\argmin}{\operatorname*{arg\,min}}

\newcommand{\lcm}{\operatorname{lcm}} % lowest common multiple
\newcommand{\Div}{\operatorname{div}} % original definition of \div

%% sets
\newcommand{\Rset}{\mathbb{R}}
\newcommand{\Qset}{\mathbb{Q}}
\newcommand{\Zset}{\mathbb{Z}}
\newcommand{\Nset}{\mathbb{N}}
\newcommand{\Znset}{\mathbb{Z}\sb{n}} % \sb instead of _ so it's ok with tex4ht
\newcommand{\Cset}{\mathbb{C}}

%% integrals, limits, brackets
\newcommand{\intinfs}{\int_{-\infty}^\infty\!\!\!}
\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}

% generic left right delimiters
% #1=size (0=unspecified) #2=left delim #3=right delim #4=contents
\newcommand{\glrdelim}[4]
%{\ifcase#1\left\or\or\bigl\or\Bigl\or\biggl\or\Biggl\fi#2#4%
%\ifcase#1\right\or\or\bigr\or\Bigr\or\biggr\or\Biggr\fi#3}
% above doesn't work maybe because \bigl etc must be next to ( etc
{\ifcase#1\left#2\or#2\or\bigl#2\or\Bigl#2\or\biggl#2\or\Biggl#2\fi%
#4\ifcase#1\right#3\or#3\or\bigr#3\or\Bigr#3\or\biggr#3\or\Biggr#3\fi}

\newcommand{\av}[1]{\langle#1\rangle}
\newcommand{\sav}[1]{\langle#1\rangle}  % for backwards compatibility
\newcommand{\lrp}[2][0]{\glrdelim{#1}{(}{)}{#2}} % left-right parentheses 
\newcommand{\lrs}[2][0]{\glrdelim{#1}{[}{]}{#2}} % left-right square brackets
\newcommand{\lrb}[2][0]{\glrdelim{#1}{\{}{\}}{#2}} % left-right braces
\newcommand{\lrm}[2][0]{\glrdelim{#1}{\lvert}{\rvert}{#2}} % left-right mod 
\newcommand{\lrn}[2][0]{\glrdelim{#1}{\lVert}{\rVert}{#2}} % left-right norm 
\newcommand{\lra}[2][0]{\glrdelim{#1}{\langle}{\rangle}{#2}}
\newcommand{\lrc}[2][0]{\glrdelim{#1}{\lceil}{\rceil}{#2}} % left-right ceil
\newcommand{\ceil}[1]{\lceil#1\rceil} % ceil
\newcommand{\lrf}[2][0]{\glrdelim{#1}{\lfloor}{\rfloor}{#2}} %  floor
\newcommand{\floor}[1]{\lfloor#1\rfloor} %  floor

%% norms
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\sabs}[1]{\lvert#1\rvert} % for backwards compatibility
\newcommand{\snorm}[2][]{\lVert#2\rVert_{#1}} % for backwards compatibility


%% functions and constants
% hspace in \e definition is needed to get spacing right after next -
\newcommand{\e}{\operatorname{e}\hspace{-0.15em}} % base of natural logs
\newcommand{\ii}{\mathrm{i}} % imaginary i 
\renewcommand{\ij}{\mathrm{j}} % imaginary j % \ij already defined

\newcommand{\degC}{$\,^\circ$C} % degrees C
%\newcommand{\degC}{\,\textdegree C} % degrees C e.g. 37\degC
%\newcommand{\nsdegC}{\textdegree C} % no space degrees C e.g. (\nsdegC)

\providecommand{\operatorname}[1]{\mathop{\mathrm{#1}}\nolimits}
\newcommand{\Res}{\operatorname{Res}} % residue
\renewcommand{\Re}{\operatorname{Re}} % real part
\renewcommand{\Im}{\operatorname{Im}} % imaginary part 
\newcommand{\Arg}{\operatorname{Arg}} % principal argument
\newcommand{\Log}{\operatorname{Log}} % principal log
\newcommand{\Ln}{\operatorname{Ln}} % principal log
\newcommand{\sgn}{\operatorname{sgn}} % sign
\newcommand{\sech}{\operatorname{sech}}
\newcommand{\cosech}{\operatorname{cosech}}
\newcommand{\cosec}{\operatorname{cosec}}
\newcommand{\sinc}{\operatorname{sinc}} % sinc(x) = sin(x) / x 
\newcommand{\erf}{\operatorname{erf}} % error function
\newcommand{\erfc}{\operatorname{erfc}} % complementary error function
\newcommand{\tr}{\operatorname{tr}} % trace
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\adj}{\operatorname{adj}} % adjugate (classical adjoint)
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\spec}{\operatorname{spec}} % spectrum
\newcommand{\Det}{\operatorname{Det}} % determinant
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\Int}{\operatorname{int}} % interior
\newcommand{\ext}{\operatorname{ext}} % exterior
\newcommand{\mes}{\operatorname{mes}} % measure

%% matrices
\newcommand{\bpm}{\begin{pmatrix}} % matrix
\newcommand{\epm}{\end{pmatrix}}
\newcommand{\bvm}{\begin{vmatrix}} % determinant
\newcommand{\evm}{\end{vmatrix}}

\newcommand{\phM}{\phantom{\ensuremath{-}}}	%minus


%% relations 
\renewcommand{\ll}{\!<\!\!<\!} % much less than
\renewcommand{\gg}{\!>\!\!>\!} % much greater than
\ifx\leqslant\undefined
\else
  \renewcommand{\leq}{\leqslant}
  \renewcommand{\geq}{\geqslant}
  \renewcommand{\le}{\leqslant}
  \renewcommand{\ge}{\geqslant}
\fi

%% words
\providecommand{\text}[1]{\mbox{#1}}
\newcommand{\prog}[1]{\textsc{#1}} % name of commercial software

% standard state symbol (from p.104 symbols-a4.pdf 2009)
\makeatletter
\providecommand\barcirc{\mathpalette\@barred\circ}
\def\@barred#1#2{\ooalign{\hfil$#1-$\hfil\cr\hfil$#1#2$\hfil\cr}}
\newcommand\stst{^{\protect\barcirc}}
\makeatother


